A survey of active galaxies at TeV photon energies with the HAWC gamma-ray observatory

The High Altitude Water Cherenkov Gamma-Ray Observatory (HAWC) continuously detects TeV photons and particles within its large field-of-view, accumulating every day a deeper exposure of two thirds of the sky. We analyzed 1523~days of HAWC live data acquired over four and a half years, in a follow-up analysis of {138} nearby ($z<0.3$) active galactic nuclei from the {\em Fermi} 3FHL catalog culminating within $40^\circ$ of the zenith at Sierra Negra, the HAWC site. This search for persistent TeV emission used a maximum-likelihood analysis assuming intrinsic power-law spectra attenuated by pair production of gamma-ray photons with the extragalactic background light. HAWC clearly detects persistent emission from Mkn~421 and Mkn~501, the two brightest blazars in the TeV sky, at 65$\sigma$ and 17$\sigma$ level, respectively. {Weaker evidence for long-term emission is found for three other known very-high energy emitters:} the radiogalaxy M87 and the BL Lac objects VER~J0521+211 and 1ES~1215+303, the later two at $z\sim 0.1$. We find evidence for collective emission from the set of 30 previously reported very high-energy sources that excludes Mkn~421 and Mkn~501 with a random probability $\sim 10^{-5}$. Upper limits are presented for the sample under the power-law assumption and in the predefined (0.5-2.0), (2.0-8.0) and (8.0-32.0) TeV energy intervals.

==> authors041b.tex <==
\author[0000-0003-0197-5646]{A.~Albert}
 \affiliation{Physics Division, Los Alamos National Laboratory, Los Alamos, NM, USA}
\author{C.~Alvarez}
 \affiliation{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}
\author{J.R.~Angeles~Camacho}
 \affiliation{Instituto de F\'{\i}sica, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author{J.C.~Arteaga-Vel\'azquez}
 \affiliation{Universidad Michoacana de San Nicol\'as de Hidalgo, Morelia, M\'exico}
\author{K.P.~Arunbabu}
 \affiliation{Instituto de Geof\'{\i}sica, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author{D.~Avila~Rojas}
 \affiliation{Instituto de F\'{\i}sica, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author[0000-0002-2084-5049]{H.A.~Ayala~Solares}
 \affiliation{Department of Physics, Pennsylvania State University, University Park, PA, USA}
\author[0000-0003-0477-1614]{V.~Baghmanyan}
 \affiliation{Institute of Nuclear Physics Polish Academy of Sciences, PL-31342 IFJ-PAN, Krakow, Poland}
\author[0000-0002-1114-2640]{E.~Belmont-Moreno}
 \affiliation{Instituto de F\'{\i}sica, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author[0000-0001-5537-4710]{S.Y.~BenZvi}
\affiliation{Department of Physics \& Astronomy, University of Rochester, Rochester, NY , USA} 
\author[0000-0002-5493-6344]{C.~Brisbois}
 \affiliation{Department of Physics, University of Maryland, College Park, MD, USA}
\author[0000-0002-4042-3855]{K.S.~Caballero-Mora}
 \affiliation{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}
\author[0000-0003-2158-2292]{T.~Capistr\'an}
 \affiliation{Instituto Nacional de Astrof\'{\i}sica, \'Optica y Electr\'onica, Tonantzintla, Puebla, M\'exico}
\author[0000-0002-8553-3302]{A.~Carrami\~nana}
 \affiliation{Instituto Nacional de Astrof\'{\i}sica, \'Optica y Electr\'onica, Tonantzintla, Puebla, M\'exico}
\author[0000-0002-6144-9122]{S.~Casanova}
 \affiliation{Institute of Nuclear Physics Polish Academy of Sciences, PL-31342 IFJ-PAN, Krakow, Poland}
\author[0000-0002-7607-9582]{U.~Cotti}
 \affiliation{Universidad Michoacana de San Nicol\'as de Hidalgo, Morelia, M\'exico}
\author[0000-0002-1132-871X]{J.~Cotzomi}
\affiliation{Facultad de Ciencias F\'{\i}sico Matem\'aticas, Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}
\author[0000-0002-7747-754X]{S.~Couti\~no~de~Le\'on}
 \affiliation{Instituto Nacional de Astrof\'{\i}sica, \'Optica y Electr\'onica, Tonantzintla, Puebla, M\'exico}
\author[0000-0001-9643-4134]{E.~De~la~Fuente}
 \affiliation{Departamento de F\'{\i}sica, Centro Universitario de Ciencias Exactas e Ingenier\'{\i}as, Universidad de Guadalajara, Guadalajara, M\'exico}
\author[0000-0001-8451-7450]{B.L.~Dingus}
 \affiliation{Physics Division, Los Alamos National Laboratory, Los Alamos, NM, USA}
\author[0000-0002-2987-9691]{M.A.~DuVernois}
 \affiliation{Department of Physics, University of Wisconsin-Madison, Madison, WI, USA}
\author{M.~Durocher}
 \affiliation{Physics Division, Los Alamos National Laboratory, Los Alamos, NM, USA}
\author[0000-0002-0087-0693]{J.C.~D\'{\i}az-V\'elez}
 \affiliation{Departamento de F\'{\i}sica, Centro Universitario de Ciencias Exactas e Ingenier\'{\i}as, Universidad de Guadalajara, Guadalajara, M\'exico}
\author[0000-0001-5737-1820]{K.~Engel}
\affiliation{Department of Physics, University of Maryland, College Park, MD, USA} 
\author[0000-0001-7074-1726]{C.~Espinoza}
 \affiliation{Instituto de F\'{\i}sica, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author{K.L.~Fan}
 \affiliation{Department of Physics, University of Maryland, College Park, MD, USA}
\author{M.~Fern\'andez~Alonso}
 \affiliation{Department of Physics, Pennsylvania State University, University Park, PA, USA}
\author[0000-0002-0794-8780]{H.~Fleischhack}
 \affiliation{Department of Physics, Michigan Technological University, Houghton, MI, USA}
\author[0000-0002-0173-6453]{N.~Fraija}
 \affiliation{Instituto de Astronom\'{\i}a, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author{A.~Galv\'an-G\'amez}
 \affiliation{Instituto de Astronom\'{\i}a, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author{D.~Garc\'{\i}a}
 \affiliation{Instituto de F\'{\i}sica, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author[0000-0002-4188-5584]{J.A.~Garc\'{\i}a-Gonz\'alez}
 \affiliation{Instituto de F\'{\i}sica, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author[0000-0003-1122-4168]{F.~Garfias}
 \affiliation{Instituto de Astronom\'{\i}a, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author[0000-0002-5209-5641]{M.M.~Gonz\'alez}
 \affiliation{Instituto de Astronom\'{\i}a, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author[0000-0002-9790-1299]{J.A.~Goodman}
 \affiliation{Department of Physics, University of Maryland, College Park, MD, USA}
\author[0000-0001-9844-2648]{J.P.~Harding}
 \affiliation{Physics Division, Los Alamos National Laboratory, Los Alamos, NM, USA}
\author[0000-0002-2565-8365]{S.~Hern\'andez}
 \affiliation{Instituto de F\'{\i}sica, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author{B.~Hona}
 \affiliation{Department of Physics, Michigan Technological University, Houghton, MI, USA}
\author[0000-0002-3808-4639]{D.~Huang}
 \affiliation{Department of Physics, Michigan Technological University, Houghton, MI, USA}
\author[0000-0002-5527-7141]{F.~Hueyotl-Zahuantitla}
 \affiliation{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}
\author{P.~H\"untemeyer}
 \affiliation{Department of Physics, Michigan Technological University, Houghton, MI, USA}
\author[0000-0001-5811-5167]{A.~Iriarte}
 \affiliation{Instituto de Astronom\'{\i}a, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author[0000-0002-6738-9351]{A.~Jardin-Blicq}
\affiliation{Max-Planck Institute for Nuclear Physics, 69117 Heidelberg, Germany}
\affiliation{Department of Physics, Faculty of Science, Chulalongkorn University, 254 Phayathai Road,Pathumwan, Bangkok 10330, Thailand}
\affiliation{National Astronomical Research Institute of Thailand (Public Organization), Don Kaeo, MaeRim, Chiang Mai 50180, Thailand}
\author[0000-0003-4467-3621]{V.~Joshi}
 \affiliation{Erlangen Centre for Astroparticle Physics, Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg, Erlangen, Germany}
 \author[0000-0003-4785-0101]{D.~Kieda}
\affiliation{Department of Physics and Astronomy, University of Utah, Salt Lake City, UT, USA}
\author[0000-0001-6336-5291]{A.~Lara}
\affiliation{Instituto de Geof\'{\i}sica, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author[0000-0002-2467-5673]{W.H.~Lee}
\affiliation{Instituto de Astronom\'{\i}a, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author[0000-0001-5516-4975]{H.~Le\'on~Vargas}
 \affiliation{Instituto de F\'{\i}sica, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
 \author[0000-0003-2696-947X]{J.T.~Linnemann}
\affiliation{Department of Physics and Astronomy, Michigan State University, East Lansing, MI, USA}
\author[0000-0001-8825-3624]{A.L.~Longinotti}
 \affiliation{Instituto Nacional de Astrof\'{\i}sica, \'Optica y Electr\'onica, Tonantzintla, Puebla, M\'exico}
\author[0000-0003-2810-4867]{G.~Luis-Raya}
 \affiliation{Universidad Polit\'ecnica de Pachuca, Pachuca, Hidalgo, M\'exico}
\author{J.~Lundeen}
 \affiliation{Department of Physics and Astronomy, Michigan State University, East Lansing, MI, USA}
\author[0000-0001-8088-400X]{K.~Malone}
 \affiliation{Physics Division, Los Alamos National Laboratory, Los Alamos, NM, USA}
\author[0000-0001-9052-856X]{O.~Mart\'{\i}nez}
\affiliation{Facultad de Ciencias F\'{\i}sico Matem\'aticas, Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}
\author[0000-0001-9035-1290]{I.~Martinez-Castellanos}
\affiliation{Department of Physics, University of Maryland, College Park, MD, USA}
\author[0000-0002-2824-3544]{J.~Mart\'{\i}nez-Castro}
 \affiliation{Centro de Investigaci\'on en Computaci\'on, Instituto Polit\'ecnico Nacional, Ciudad de M\'exico, M\'exico}
\author[0000-0002-2610-863X]{J.A.~Matthews}
 \affiliation{Dept of Physics and Astronomy, University of New Mexico, Albuquerque, NM, USA}
\author[0000-0002-8390-9011]{P.~Miranda-Romagnoli}
 \affiliation{Universidad Aut\'onoma del Estado de Hidalgo, Pachuca, M\'exico}
 \author{J.A.~Morales-Soto}
\affiliation{Universidad Michoacana de San Nicol\'as de Hidalgo, Morelia, M\'exico}
\author[0000-0002-1114-2640]{E.~Moreno}
 \affiliation{Facultad de Ciencias F\'{\i}sico Matem\'aticas, Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}
\author[0000-0002-7675-4656]{M.~Mostaf\'a}
 \affiliation{Department of Physics, Pennsylvania State University, University Park, PA, USA}
\author[0000-0003-0587-4324]{A.~Nayerhoda}
 \affiliation{Institute of Nuclear Physics Polish Academy of Sciences, PL-31342 IFJ-PAN, Krakow, Poland}
\author[0000-0003-1059-8731]{L.~Nellen}
 \affiliation{Instituto de Ciencias Nucleares, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author[0000-0001-9428-7572]{M.~Newbold}
 \affiliation{Department of Physics and Astronomy, University of Utah, Salt Lake City, UT, USA}
\author[0000-0002-0479-2311]{M.U.~Nisa}
 \affiliation{Department of Physics and Astronomy, Michigan State University, East Lansing, MI, USA}
\author[0000-0001-7099-108X]{R.~Noriega-Papaqui}
 \affiliation{Universidad Aut\'onoma del Estado de Hidalgo, Pachuca, M\'exico}
\author{L.~Olivera-Nieto}
\affiliation{Max-Planck Institute for Nuclear Physics, 69117 Heidelberg, Germany}
\author{A.~Peisker}
 \affiliation{Department of Physics and Astronomy, Michigan State University, East Lansing, MI, USA}
\author[0000-0001-5998-4938]{E.G.~P\'erez-P\'erez}
 \affiliation{Universidad Polit\'ecnica de Pachuca, Pachuca, Hidalgo, M\'exico}
\author[0000-0002-6524-9769]{C.D.~Rho}
 \affiliation{University of Seoul, Seoul, Rep. of Korea}
\author[0000-0003-1327-0838]{D.~Rosa-Gonz\'alez}
 \affiliation{Instituto Nacional de Astrof\'{\i}sica, \'Optica y Electr\'onica, Tonantzintla, Puebla, M\'exico}
\author[0000-0001-6939-7825]{E.~Ruiz-Velasco}
\affiliation{Max-Planck Institute for Nuclear Physics, 69117 Heidelberg, Germany}
\author{H.~Salazar}
 \affiliation{Facultad de Ciencias F\'{\i}sico Matem\'aticas, Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}
\author[0000-0002-8610-8703]{F.~Salesa~Greus}
\affiliation{Institute of Nuclear Physics Polish Academy of Sciences, PL-31342 IFJ-PAN, Krakow, Poland}
\affiliation{Instituto de F\'{\i}sica Corpuscular, CSIC, Universitat de Val\'{e}ncia, E-46980, Paterna, Valencia, Espa\~na}
\author[0000-0001-6079-2722]{A.~Sandoval}
 \affiliation{Instituto de F\'{\i}sica, Universidad Nacional Aut\'onoma de M\'exico, Ciudad de M\'exico, M\'exico}
\author[0000-0001-8644-4734]{M.~Schneider}
 \affiliation{Department of Physics, University of Maryland, College Park, MD, USA}
\author[0000-0002-8999-9249]{H.~Schoorlemmer}
\affiliation{Max-Planck Institute for Nuclear Physics, 69117 Heidelberg, Germany}
\author[0000-0002-1012-0431]{A.J.~Smith}
\affiliation{Department of Physics, University of Maryland, College Park, MD, USA}
\author[0000-0002-1492-0380]{R.W.~Springer}
 \affiliation{Department of Physics and Astronomy, University of Utah, Salt Lake City, UT, USA}
\author[0000-0001-9725-1479]{K.~Tollefson}
 \affiliation{Department of Physics and Astronomy, Michigan State University, East Lansing, MI, USA}
\author[0000-0002-1689-3945]{I.~Torres}
 \affiliation{Instituto Nacional de Astrof\'{\i}sica, \'Optica y Electr\'onica, Tonantzintla, Puebla, M\'exico}
\author{R.~Torres-Escobedo}
 \affiliation{Departamento de F\'{\i}sica, Centro Universitario de Ciencias Exactas e Ingenier\'{\i}as, Universidad de Guadalajara, Guadalajara, M\'exico}
\author{F.~Ure\~na-Mena}
 \affiliation{Instituto Nacional de Astrof\'{\i}sica, \'Optica y Electr\'onica, Tonantzintla, Puebla, M\'exico}
\author[0000-0001-6876-2800]{L.~Villase\~nor}
 \affiliation{Facultad de Ciencias F\'{\i}sico Matem\'aticas, Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}
\author{T.~Weisgarber}
 \affiliation{Department of Chemistry and Physics, California University of Pennsylvania, California, Pennsylvania, USA}
 \author{E.~Willox}
\affiliation{Department of Physics, University of Maryland, College Park, MD, USA} 
\author[0000-0001-9976-2387]{A.~Zepeda}
 \affiliation{Departamento de F\'{\i}sica, Centro de Investigaci\'on y de Estudios Avanzados del IPN, Ciudad de M\'exico, M\'exico}
\author[0000-0003-0513-3841]{H.~Zhou}
 \affiliation{Tsung-Dao Lee Institute \&{} School of Physics and Astronomy, Shanghai Jiao Tong University, Shanghai, China}
\author[0000-0002-8528-9573]{C.~de Le\'on}
 \affiliation{Universidad Michoacana de San Nicol\'as de Hidalgo, Morelia, M\'exico}

